Fundamental Limits of Age-of-Information in Stationary and Non-stationary Environments

We study the multi-user scheduling problem for minimizing the Age of Information (AoI) in cellular wireless networks under stationary and non-stationary regimes. We derive fundamental lower bounds for the scheduling problem and design efficient online policies with provable performance guarantees. In the stationary setting, we consider the AoI optimization problem for a set of mobile users travelling around multiple cells. In this setting, we propose a scheduling policy and show that it is $2$-optimal. Next, we propose a new adversarial channel model for studying the scheduling problem in non-stationary environments. For $N$ users, we show that the competitive ratio of any online scheduling policy in this setting is at least $\Omega(N)$. We then propose an online policy and show that it achieves a competitive ratio of $O(N^2)$. Finally, we introduce a relaxed adversarial model with channel state estimations for the immediate future. We propose a heuristic model predictive control policy that exploits this feature and compare its performance through numerical simulations.

==> improved_lower_bound.tex <==
\section{A tight universal lower bound} 
%It can be seen that, if we use the general lower bound for the stochastic problem as given in Theorem \ref{uni_lb}, we obtain a vacuous competitive ratio of $1$. In this Section, with a tighter analysis of the symmetric $2$ user stochastic problem, we obtain a lower bound to the competitive ratio of value $ 1.5$.  
%Note that, for applying Yao's principle, it is enough to restrict our attention to the deterministic online policies only \cite{motwani1995randomized}. \\
In this section, we derive an improved universal lower bound for a single BS in which only one user may be scheduled among $N$ users at a slot. For simplicity, we assume that the UEs have statistically identical channels, \emph{i.e.,} $p_i=p, \forall 1\leq i \leq N$. \\
Let $\mathcal{F}_{t}\equiv \sigma(\vec{h}(k), \vec{\mu}(k), 1\leq k \leq t)$ be the sigma-algebra generated by the random age $\vec{h}(t)$ and scheduling decisions $\vec{\mu}(t)$ up to time $t$. For any online policy, the scheduling decision $\vec{\mu}(t+1)$ at the beginning of the slot $t+1$ must be measurable in the sigma-algebra $\mathcal{F}_{t}$.  Let the random variable $H_{\textrm{sum}}(t) \equiv (\sum_i h_i(t))$ denote the sum of ages of all UEs at time $t$. Let $B_i(t) \in \mathcal{F}_t$ be the event under which the policy $\pi$ schedules the $\textrm{UE}_i, \forall i$.  Clearly, $B_i(t) \cap B_j(t)=\phi, \forall i\neq j$ and $\sqcup_i B_{i}(t)=\Omega.$ 
%and $Q(t)= \prod_{i=1}^{N}H_i(t)$. WOLOG, let's assume that, given the information up to time $t$, the online policy schedules the $j$\textsuperscript{th} UE at time $t$.  
%Consider the following two exhaustive and mutually exclusive cases:
%\paragraph{Case I: The online policy $\pi$ schedules the $\textrm{UE}_1$ at time $t$.} 
%In this case, we have the following: 
Hence, we can write 
\begin{eqnarray*}
%\mathbb{E}\big(h_i(t+1)| \mathcal{F}_{t}\big) = \begin{cases}
% 1+ h_i(t), ~~\textrm{if} ~i\neq j\\
% 1+ \bar{p}h_i(t), ~~\textrm{if} ~ i=j,	
% \end{cases}
\mathbb{E}\big(h_i(t+1)| \mathcal{F}_{t}\big) &=& \mathds{1}(B_i(t))\big(p + (1-p)(1+h_i(t)\big)\\
 &&+ \mathds{1}(B_i^c(t))\big(1+h_i(t)\big)\\
 &=& 1+ h_i(t) - p h_i(t) \mathds{1}(B_i(t)).  
\end{eqnarray*}
Hence,
\begin{eqnarray*}
\mathbb{E}(H_{\textrm{sum}}(t+1)| \mathcal{F}_t)= N+ H_{\textrm{sum}}(t) - p \sum_{i}h_i(t)\mathds{1}(B_i(t)).	
\end{eqnarray*}
Next, we define the set of exhaustive and mutually exclusive events $\{B_i'(t)\}_{i}$ as follows:
\begin{eqnarray*}
	B_i'(t) = \{ \omega \in \Omega: h_i(t, \omega) \geq h_j(t, \omega), \forall j \neq i\},
\end{eqnarray*}
where, in the above, we break ties uniformly at random. Then, it follows that 
\begin{eqnarray*}
\mathbb{E}(H_{\textrm{sum}}(t+1)| \mathcal{F}_t) &\geq& N+ H_{\textrm{sum}}(t) - p \sum_{i}h_i(t)\mathds{1}(B_i'(t))\\
	&=& N+ H_{\textrm{sum}}(t) - p h_{\max}(t).
\end{eqnarray*}
It is clear that, 


%where $\bar{p}\equiv 1-p$. Taking expectation of both sides, we have 
%\begin{eqnarray*}
%H_i(t+1) = \begin{cases}
% 1+ H_i(t), ~~\textrm{if} ~i\neq j\\
% 1+ \bar{p}H_i(t), ~~\textrm{if} ~ i=j.	
% \end{cases}
%\end{eqnarray*}
%Hence,
%\begin{eqnarray*}
%&&Q(t+1) \\
%&\equiv& \prod_{i=1}^{N}H_i(t+1) \\
%&=&  (1+ \bar{p}H_j(t))\prod_{i=1, i\neq j}^{N} \big(1+H_i(t)\big)\\
%&=& (1+ \bar{p}H_j(t)) \bigg(1 + \sum_{k=1}^{N-1}\prod_{i \in S:|S|=k, j\notin S} H_i(t) \bigg) 
%\end{eqnarray*}
%where the last inequality follows from the fact that $H_2(t)\geq 1$ and an application of the AM-GM inequality. 
%\paragraph{Case II: The online policy $\pi$ schedules the $\textrm{UE}_2$ at time $t$}
%Using a symmetric argument, it can be proved that even in this case, we have the inequality
%\begin{eqnarray} \label{p_ineq}
%	p(t+1) \geq \frac{3}{2}+ \frac{1}{2}p(t) + \sqrt{p(t)}.
%\end{eqnarray}

%Note that, the asymptotic time-averaged AoI of the scheduling policy $\pi$ is lower bounded as follows:
%
%\begin{eqnarray} \label{lim_cost}
%\liminf_{T\to \infty}\frac{1}{T}\mathbb{E}(C_T(\pi)) &=& \liminf_{T\to \infty} \frac{1}{T}\sum_{t=1}^{T} \big(H_1(t) + H_2(t)\big) \nonumber \\
%&\stackrel{\textrm{AM-GM}}{\geq}&  2 \liminf_{T\to \infty} \frac{1}{T}\sum_{t=1}^{T} \sqrt{p}(t) \nonumber \\
%&\geq & 2 \sqrt{\liminf_{T \to \infty} p(T)},	
%\end{eqnarray}
% where the last inequality follows from the Cesaro Mean Theorem \cite{williams1991probability}. From Eqn.\ \eqref{lim_cost}, it is clear that, we need to investigate the limiting properties of the recursive inequality \eqref{p_ineq}, to draw conclusion about the cost lower bound of any online policy. For this, let $L=\liminf_{T\to\infty} p(T)$, which we assume, WOLOG, to be finite. Taking $\liminf$ of both sides of \eqref{p_ineq}, we conclude
% \begin{eqnarray*}
% L \geq \frac{3}{2} + \frac{1}{2}L + \sqrt{L}.	
% \end{eqnarray*}
% i.e., $L \geq 9$. Hence, from Eqn.\ \eqref{lim_cost}, we conclude that the limiting time-averaged AoI incurred by any online policy $\pi$ is lower bounded as follows:
% \begin{eqnarray}\label{cost_lb}
% 	\liminf_{T\to \infty}\frac{1}{T}\mathbb{E}(C_T(\pi)) \geq 2 \sqrt{9}= 6.
% \end{eqnarray}
%
%Hence, combining Eqns. \eqref{opt_cost} and \eqref{cost_lb}, we conclude that the asymptotic competitive ratio $\eta_{\infty}$ of any online scheduling policy $\pi$ is lower bounded as \[\sup_{T \geq 1} \frac{\mathbb{E}(C_T(\pi))}{\mathbb{E}(C_T(\textsf{OPT}))}  \geq \liminf_{T\to \infty} \frac{\mathbb{E}(C_T(\pi))}{\mathbb{E}(C_T(\textsf{OPT}))} \geq \frac{6}{4} = 1.5.\]
%
%

